Almost Free: Self-concordance in Natural Exponential Families and an Application to Bandits

We prove that single-parameter natural exponential families with subexponential tails are self-concordant with polynomial-sized parameters. For subgaussian natural exponential families we establish an exact characterization of the growth rate of the self-concordance parameter. Applying these findings to bandits allows us to fill gaps in the literature: We show that optimistic algorithms for generalized linear bandits enjoy regret bounds that are both second-order (scale with the variance of the optimal arm's reward distribution) and free of an exponential dependence on the bound of the problem parameter in the leading term. To the best of our knowledge, ours is the first regret bound for generalized linear bandits with subexponential tails, broadening the class of problems to include Poisson, exponential and gamma bandits.

==> main/old_setting.tex <==
For any probability distribution $Q$ over the reals
and $u\in \RR$, we let $\psi_Q(u) = \log \int e^{u y} Q(dy)$ be the \emph{cumulant-generating function} of $Q$, and let $\cU_Q \subset \RR$ be the largest set  on which $\psi_Q(u)$ is finite. The natural exponential family generated by a distribution $Q$ is the family
$(Q_u(dy))_{u\in \cU_Q}$ of probability measures on $\RR$ where
\begin{equation*}
	Q_u(dy) = \frac{1}{M_Q(u)}\exp(yu) Q(dy) \spaced{for} u \in \cU_Q\,.
\end{equation*}
where $M_Q(u)=\exp(\psi_Q(u))=\int e^{u y} Q(dy)$ is the moment generating function of $Q$.
As is well known, $\cU_Q$ is always an interval.
We only consider \emph{regular} families, i.e., families where 
$\cU_Q^\circ$, the interior of $\cU_Q$, is not empty.

The Bernoulli and Gaussian distributions are examples of regular families with $\cU=\cU_Q = \RR$.
The Bernoulli distribution corresponds to the base distribution that is the uniform distribution on $\{0,1\}$, while the Gaussian distribution corresponds to $Q$ chosen as the standard normal distribution. 
The latter is a somewhat unusual choice (as opposed to choosing $Q$ to be Lebesgue measure), though this makes no difference.
\subsection{Bandit \& Regret}
We consider bandit problems described by a non-empty (possibly infinite) arm set $\cX\subset \RR^d$, a parameter vector $\theta_\star\in \Theta \subset \RR^d$, and a family of distributions $(P(\cdot;u))_{u\in \cU}$ over the reals
where $\cU\subset \RR$ is a (possibly infinite) interval of real numbers with non-empty interior such that for all $x\in \cX$, $x^\top \theta_\star\in \cU$. We will use $\mu(u)$ to denote the mean of $P(\,\cdot\,;u)$: 
\[
\mu(u) = \int y\,\, P(dy;u)\,.
\]
We consider bandit problems where the learner is given the family $(P(\,\cdot\,;u))_{u\in \cU}$, the arm set $\cX$, but not the parameter $\theta_\star$.
In each round $t \in\{1,2, \dotsc\}$ of the interaction, the learner selects an action $X_t \in \cX$
based on the available past information.
In response to the action selected, the learner receives a random reward $Y_t \in \RR$, which they observe. For the reward distribution, we assume Generalized Linear Bandit (GLB) model throughout this work, which is formalized below.
\begin{assumption}[Generalised linear bandit]
\label{ass:glb}
The rewards in our bandit instances are determined by $(P(\cdot;u))_u$  which corresponds to a natural exponential family $\cQ=(Q_u(dy))_{u\in \cU}$ generated by some base $Q$:
\begin{align*}
P(\cdot;u) = Q_u(\cdot) \spaced{for} u\in \cU\,,
\end{align*}
where $\cU = \cU_Q^\circ$ is an interval with non-empty interior. Furthermore, the distribution of $Y_t$, given the past, and in particular $X_t$, is
$P(\,\cdot\,; X_t^\top \theta_\star)$.
\end{assumption}

The goal of the learner is to maximize its mean reward. 
The performance of the learner is measured by their (pseudo)regret,
which, for an interaction that lasts for $n$ rounds, is given 
\begin{equation*}
	\regret(n) = \sum_{t=1}^n \mu(x_\star^\top \theta_\star) - \mu(X_t^\top \theta_\star)\,,
\end{equation*}
where $x_\star$ is any arm in $\argmax_{x \in \cX} \mu(x^\top \theta_\star)$.
For simplicity, we assume that such an arm exists.
We will design algorithms for the learner that rely on regularised maximum likelihood estimation,
or, equivalently, by minimising the regularised negative log-likelihood loss. 
To define the likelihood function, assume that each distribution in the family $(P(\cdot;u))_{u\in \cU}$ is dominated by a common $\sigma$-finite measure $\nu$ over the reals. This allows us to consider the density of $P(\cdot;u)$ with respect to $\nu$, which we will denote by $p(\cdot;u)$; that is,
$p(y;u)  = \frac{d P(\cdot;u)}{d\nu}$. Then, given a list of pairs $\cD = ( (X_1,Y_1),\dots,(X_s,Y_s))$ of length $s$ where $X_i\in \cX$ and $Y_i\in \RR$,
and a regularisation parameter $\lambda>0$,
the $\lambda$-regularised \emph{negative} log-likelihood function is defined to be
\begin{equation}
	\cL(\theta; \cD,\lambda) = \frac{\lambda}{2} \|\theta\|^2 -\sum_{i=1}^s \log p(Y_i; X_i^\top\theta)\,.
\end{equation}

==> main/related_work.tex <==
%!TEX root =  ../main.tex
\section{Related Work}\todoc{I would definitely move this to the end where the results have been presented.}
\paragraph{Generalized Linear Bandits}
The framework of generalized linear bandits was first introduced by \cite{Filippi2010parametric} in which the authors propose an optimistic algorithm, GLM-UCB, that gets bounded regret. \cite{pmlr-v70-li17c} proposed SupCB-GLM which achieved a regret bound being $\sqrt d$ tighter than GLM-UCB under the assumption of finite arm set. On the side of randomized algorithms, \cite{abeille2017linear} applied Thompson sampling to GLBs whose regret upper bound was later improved by a factor of $\sqrt{d/\log K}$ in \cite{kveton2019Randomized} under finite arm setting. \cite{kveton2019Randomized} also proposed GLM-FPL that fits the model to the past observed reward perturbed by Gaussian noise. The regret upper bounds of all of the above works depend linearly on $\kappa$ in the first order term. 
As a special instance of GLBs, logistic bandits have received a lot of attentions in recent years. \cite{faury2020improved} was the first one to shave off the $\kappa$ dependency in the first order term of regret upper bound by making use of the pseudo-self-concordant property of logistic function which was originally studied by \cite{Bach2010self} in logistic regression. Their analysis was later tightened by \cite{Abeille2020InstanceWiseMA} who also proved a regret lower bound to match with their upper bound. Following the pseudo-self-concordant style of analysis in \cite{faury2020improved}, \cite{russac2021self} studied GLBs that are similar to logistic bandits by assuming pseudo-self-concordant link functions and bounded reward distributions but with a focus on non-stationary environment. \cite{janz2023exploration} proposed EVILL that applied linear perturbation to loss function to solve structured bandit problems that are more general than GLBs and showed that EVILL is able to achieve performance comparable to Thompson sampling style of perturbation-based algorithms under the assumption of generalized pseudo-self-concordance and the MGF of the base distribution is defined on the reals.
\paragraph{Self-concordant functions}
Prior to GLBs, (pseudo) self-concordant functions have already been widely studied in optimization and statistical learning theory. 
Self-concordant functions classically stands for the third derivative is uniformly upper bounded by the $1.5$-th power of the second derivative, which were first introduced by \cite{Nesterov1994InteriorpointPA}. \cite{Bach2010self} studied pseudo-self-concordant property of logistic function, which removes the power condition in self-concordant functions, in the context of Newton's method. \cite{Sun2017GeneralizedSF} proposed generalized self-concordant functions which is a general framework that includes both functions mentioned above to design Newton-type of methods. \cite{Ostrovskii2020finite} developed oracle inequalities for M-estimators of both self-concordant and pseudo-self-concordant functions under mild assumptions. \cite{marteau-ferey2019beyond} showed non-asymptotic convergence rate faster than $O(1/\sqrt n)$ can be achieved for the regularized empirical risk minimizer on pseudo-self-concordant losses.

